On Failure Diagnosis of the Storage Stack

Diagnosing storage system failures is challenging even for professionals. One example is the "When Solid State Drives Are Not That Solid" incident occurred at Algolia data center, where Samsung SSDs were mistakenly blamed for failures caused by a Linux kernel bug. With the system complexity keeps increasing, such obscure failures will likely occur more often. As one step to address the challenge, we present our on-going efforts called X-Ray. Different from traditional methods that focus on either the software or the hardware, X-Ray leverages virtualization to collects events across layers, and correlates them to generate a correlation tree. Moreover, by applying simple rules, X-Ray can highlight critical nodes automatically. Preliminary results based on 5 failure cases shows that X-Ray can effectively narrow down the search space for failures.

==> background.tex <==
%\vspace{-0.1in}
%\section{Background of File System Checkers}
\section{Background}
\label{sec:background}
%%\vspace{-0.1in}
%File system checkers are designed to check and repair inconsistencies in file systems.
%Depending on the structures of file systems, the checkers may perform different number of checking passes
%and examine different consistency rules.
%We use~\texttt{e2fsck}
%%~\cite{e2fsck} %,
%, the default checker of the popular Ext-series file systems, 
%as a concrete example to illustrate the complexity as well as the potential vulnerabilities of checkers in this section.
%
%\vspace{-0.1in}
%\subsection{Workflow of~\texttt{e2fsck}}
%\label{sec:background-e2fsck}
%\vspace{-0.05in}
%The first action of \texttt{e2fsck} is to replay the journal (in case of Ext3/Ext4) and then restart itself. Next, \texttt{e2fsck} executes the following five passes in order:
%% 
%
%%\begin{itemize}
%%\begin{enumerate}
%%\textbf{Pass 1: Scan the entire file system}\\ 
%\vspace{-0.17in}
%\paragraph{Pass-1: Scan the entire file system and check inodes.}
%In this pass \texttt{e2fsck} 
%%This pass 
%iterates over all inodes and checks each inode one by one (e.g., validating the mode, size, and block count). 
%Meanwhile, it stores the scanned information in a set of bitmaps,  including inodes in use (\texttt{inode\_used\_map}), 
%%inodes with bad fields (\texttt{inode\_bad\_map}), % inodes in bad blocks (\texttt{inode\_bb\_map}),  
%%blocks in use (\texttt{block\_found\_map}), 
% blocks claimed by two inodes (\texttt{block\_dup\_map}), etc.
%%inodes representing directories and regular files (\texttt{inode\_dir\_map} and \texttt{inode\_reg\_map}),  
%% data blocks belonging to directory inodes (\texttt{dir\_map}).
%Besides, it performs four sub-passes %(Pass 1B - 1E) 
%to generate a list of duplicate blocks and their owners, checks the integrity of the extent trees, etc.
%
%\vspace{-0.17in}
%\paragraph{Pass-2: Check directory structure.}
%Based on the bitmaps collected, 
%this pass iterates through all directory inodes and checks a set of rules for each directory. 
%For example,  the first directory entry should be ``.'', 
%the length of each entry (\texttt{rec\_len}) should be within a range,
%%the inode number in the directory entry should refer to an in-use inode,
%etc.
%%In some cases, 
%%If Pass 2 is unable to add checksum to the directory leaf nodes (due to space requirements), then these directories are rebuilt in Pass 3A.
%%To reduce the disk seek time, the directory entries are processed in the sorted order of block numbers.
%
%\vspace{-0.17in}
%\paragraph{Pass-3: Check  connectivity.}
%This pass ensures that all  directories are connected properly in the file system tree. 
%To this end, \texttt{e2fsck} first checks whether a root directory exists. If not,  then a new root directory is created and is marked as ``done''. 
%Next, \texttt{e2fsck} iterates over all directory inodes and attempts to traverse up the file system tree, until it reaches a directory marked as ``done''. If no ``done'' directory is reachable, 
% the current directory inode is marked as disconnected, and \texttt{e2fsck} offers to reconnect it to the "lost+found" folder.
%During the traversal, if \texttt{e2fsck} sees a directory twice (i.e., there is a loop),
%\texttt{e2fsck} also offers to reconnect the directory to the "lost+found" folder to
%break the loop.
%%, so as to break the loop.
%%Besides, Pass 3 has a subpass called "Pass 3A", which performs directory optimization (such as indexing directory inodes and removing duplicate entries) by rebuilding the tree directories.
%% \fixme{what does optimize mean?is reconnect performed in Pass 3 or 4?}
% 
%
%\vspace{-0.17in}
%\paragraph{Pass-4: Check reference counts.}
%This pass iterates over all the inodes to validate the inode link counts.
%Also, it checks the connectivity of the extended attribute (EA) blocks and reconnects them if necessary.
%In addition, Pass-4 loads a set of readahead bitmaps for the next pass.  
%%\fixme{what are  readahead bitmaps?is reconnect performed in Pass 3 or Pass 4? Where is reference count used?}
%
%\vspace{-0.17in}
%\paragraph{Pass-5: Recalculate checksums and flush updates.}
%In the final pass, \texttt{e2fsck} checks the repaired in-memory data structures against on-disk data structures and flush necessary updates to the disk to ensure consistency. Also, if the in-memory data structures are mapped dirty due to the fixes in the previous passes, the corresponding checksums are re-calculated before flushing.
%
%
%
%%\fixme{add a short paragraph to highlight the vulnerabilities in the five passes.}
%Based on the analysis above, we can see that the workflow of~\texttt{e2fsck} is complicate and may be vulnerable to faults. 
%For example, 
%%there are cross-pass dependency (e.g., the bitmaps are used and updated by multiple passes)
%later passes may depend on previous passes
% (e.g., the bitmaps are read and updated by multiple passes), some early fixes are not committed until the last pass, 
% and there is no atomicity guarantee for related updates. 
%We describe our method for systematically exposing the vulnerabilities %in the next section.
%in~\S\ref{sec:testing}.
%
%
%\begin{figure*}[tb] 
%\centering
%\includegraphics[width=6.2in]{./figure/workflow.pdf}
%\vspace{-0.15in}
%\caption{
%{\bf (a) Testing the fault resilience of a file system checker (fsck).} 
%{\it
%%(a)~\texttt{fsck} without logging support.
%There are ten steps: 
%(1) make a copy of the test image which contains a corrupted file system;
%(2) run {fsck} on the copy of test image;
%(3) store the image generated in step 2 as the reference image;
%(4) record the I/O commands generated during the {fsck};
%(5) make another copy of the test image;
%(6) replay partial commands to emulate the effect of an interrupted {fsck} on the copy of test image;
%(7) store the image generated in step 6 as the interrupted image;
%(8) run {fsck} on the interrupted image;
%(9) store the image generated in step 8 as the repaired image;
%(10) compare  the repaired image with the reference image to identify mismatches.
%}
%{\bf (b) Testing fsck with logging support.}
%{\it The workflow is similar except that the fault injection module interrupts the I/O commands
%sent to both the test image and the log, and the log is replayed between steps 7 and 8.
%}
%}
%\vspace{-0.1in}
%\label{fig:workflow} 
%\end{figure*}
%
%\vspace{-0.1in}
%\subsection{The {undo} logging of~\texttt{e2fsck}}
%\label{sec:background-undo}
%\vspace{-0.05in}
%Some file system developers have envisioned the potential  need of reverting  the changes done to the file system.
%For example, the ``undo io manager'' has been added to~\texttt{e2fsprogs}~\cite{e2fsprogs} since 2007~\cite{undo_io},
%which can save the content of the location being overwritten to an undo log before committing the overwrite.
%
%
%However, due to the degraded performance as well as the log format issues~\cite{Ted,ditch_tdb_file}, 
%the {undo} feature has not been integrated into~\texttt{e2fsck} until recently.
%%cannot be enabled by the user directly%through the command line option of~\texttt{e2fsck} 
%%until 2015~\cite{option}.
%Starting from v1.43, \texttt{e2fsck} includes a ``-z'' option to allow the user to specify the path of the log file and enable logging~\cite{e2fsprogs}. 
%%When enabled,~\texttt{e2fsck} creates an undo log  before any passes. %\fixme{Om: verify}. 
%%During the checking, it  %asynchronously 
%When enabled, \texttt{e2fsck} maintains an undo log during the checking, and
%writes an undo block to the log  before updating any block of the image. 
%%At the end of the last pass, it flushes all buffered writes to the file system image as well as the log file. %, respectively.
%If~\texttt{e2fsck} fails unexpectedly, the undo log can be replayed via~\texttt{e2undo}~\cite{e2fsprogs} to revert the undesired changes. 
%%, which essentially provides a write ahead logging (WAL) mechanism for the file system utilities including~\texttt{e2fsck}. % in ~\texttt{e2fsprogs}.
%
%%Since the undo logging saves the original content, one might expect that it can prevent any unrecoverable corruptions caused by an interrupted~\texttt{e2fsck}. 
%%As we will demonstrate in \S\ref{sec:testing}, however, this is not true.
%%As we will see in the next section, however, this is not true.
%Given the undo logging, one might expect that an interrupted \texttt{e2fsck} will not cause any issue.
%As we will see in the next section, however, this is not true.


==> case-fdatasync.tex <==



\vspace{-0.1in}
\subsection{Case Study II: \texttt{ext4\_sync\_file}}
\label{sec:case-fdatasync}
\vspace{-0.05in}





\subsubsection{Failure Symptom}
\vspace{-0.05in}
The failure symptom is that 
when only the size of a file is changed,
calling \texttt{fdatasync} does not persist the size update, so the file may have a wrong size after crash.



\vspace{-0.05in}

\subsubsection{Diagnosis}
\vspace{-0.05in}

Similar to the previous case (\S\ref{sec:case-fsync}),
%We run a  workload simplified from the one described in ~\cite{Zheng-TOCS16-SSD}.
we use two normal systems for reference to demonstrate the stability:
%We compare the abnormal system with two normal systems: 
one system differs from the abnormal system (v4.15.0) by only one  patch,
and the other is multiple major releases apart (v5.0.0).
As shown in Figure~\ref{fig:casefdatasync}, 
the \texttt{fdatasync} call leads to 
different device commands: one ``cmd:WRITE" and  one
``cmd:SYNC\_CACHE" in Figure~\ref{fig:casefdatasync}a, but multiple commands in \ref{fig:casefdatasync}b and \ref{fig:casefdatasync}c. By annotating the trees with syscall markers and comparing across abnormal/normal systems, we can identify the root of divergence  (``ext4\_fsync\_file'').
The paths on Figure~\ref{fig:casefdatasync}b and ~\ref{fig:casefdatasync}c are the same in this example, and are equally effective for narrowing down the root cause. 
%In this case we reduce the search space from 995 nodes to  27 nodes.


\vspace{-0.05in}

\subsubsection{Root Cause}
\vspace{-0.05in}

%when only inode's \texttt{i\_size} is changed.
The root cause is that Ext4 does not track the 
inode \texttt{i\_size} update properly. 
As a result, \texttt{ext4\_sync\_file} dose not 
include the size update into 
a journal transaction under the \texttt{fdatasync} call.


==> case-fsync.tex <==
\vspace{-0.1in}

\subsection{Case Study I: \texttt{blkdev\_fsync}}
\label{sec:case-fsync}
\vspace{-0.05in}


\begin{figure*}[tb]
    \begin{center}
           \includegraphics[width=\textwidth]{./figure/casefsync.png}
    \end{center}
    \vspace{-0.3in}
    \caption{
        {\bf Example Report of Case Study I (\S\ref{sec:case-fsync})}. 
        {\it (a) The suspicious path on the abnormal system; 
       (b) the reference path on a normal system with 1 patch difference; 
       (c) the reference path on another normal system with more than XXX patches difference. 
       The shaded nodes are the syscall markers (``syscall:fsync'') and 
       command markers (``cmd:WRITE'' and ``cmd:SYNC\_CACHE''); 
       the bold function (``blkdev\_fsync'') is identified as the root of divergence.}
    }
    \label{fig:casefsync}
\end{figure*}



\subsubsection{Failure Symptom}
\label{sec:fsync}
\vspace{-0.05in}

This is one of the two cases mentioned in \S\ref{sec:intro}~\cite{Zheng-TOCS16-SSD}. 
The failure symptom 
is that some ``committed'' synchronous writes to a raw block device are not persisted on the device,
and thus may appear to be lost after power faults.

%\subsubsection{Workload}
%\label{sec:fsync-wkld}
\vspace{-0.1in}

\subsubsection{Diagnosis}
\label{sec:fsync-diagnosis}
\vspace{-0.05in}

%We run a  workload simplified from the one described in ~\cite{Zheng-TOCS16-SSD}.
The abnormal system is based on Linux kernel v4.15.0.
%To demonstrate the effectiveness, 
We compare the abnormal system with two normal systems: 
the first one  differs from the abnormal version by only one kernel patch (i.e., the path that fixed the bug);
the second one  is multiple major releases apart (v5.0.0),
and differs by about  10,168 patches.
These two normal systems represent two  extreme cases for comparison.


Figure~\ref{fig:casefsync} shows a simplified report from \texttt{VDB}.  
We can see that one \texttt{fsync}  call generates different device commands: ``cmd:WRITE'' on the abnormal system (Figure~\ref{fig:casefsync}a);  ``cmd:WRITE'' and  ``cmd:SYNC\_CACHE'' on normal systems (\ref{fig:casefsync}b and \ref{fig:casefsync}c).
Figure~\ref{fig:casefsync}a shows the suspicious path 
on the abnormal system based on the syscall marker (``syscall:fsync'') and command markers (``cmd:WRITE''). 
Similarly, \ref{fig:casefsync}b and \ref{fig:casefsync}c show the corresponding paths from the two normal systems, respectively.
By comparing across traces, 
we can identify the root of divergence
 (``blkdev\_fsync'').
Also, we can see that \ref{fig:casefsync}b and  \ref{fig:casefsync}c are  equally helpful for reducing the search space of root cause from 
the entire call tree to a few branches.
In other words,
\texttt{VDB} is effective even if we use a reference system 
that is much different from the target abnormal system.  

 
% reducing the search space from XXX nodes to  25 nodes, respectively.   

\vspace{-0.1in}

\subsubsection{Root Cause}
\label{sec:fsync-diagnosis}
\vspace{-0.05in}

Based on the report of \texttt{VDB}, the root cause is 
easy to pinpoint. Essentially, 
the barrier support in {blkdev\_fsync} is broken.
%the block device code of the kernel is missing (i.e., \texttt{blkdev\_fsync} is broken). 
As a result, when the user workload 
invokes \texttt{fsync} 
on a block device (which eventually invokes 
\texttt{blkdev\_fsync}), there is no guarantee that a flush cache command is sent to the device.
%In other words, the failure (i.e.,  lost writes after power faults) 
%is not caused by a misbehaved device.


\begin{figure*}[tb]
    \begin{center}
           \includegraphics[width=\textwidth]{./figure/casefdatasync.png}
    \end{center}
    \vspace{-0.3in}
    \caption{
         {\bf Example Report of Case Study II (\S\ref{sec:case-fdatasync})}. 
        {\it (a) The suspicious path on the abnormal system; 
       (b) the reference path on a normal system with 1 patch difference; 
       (c) the reference path on another normal system with more than XXX patches difference. 
       The shaded nodes are the syscall markers (``syscall:fdatasync'') and 
       command markers (``cmd:WRITE'' and ``cmd:SYNC\_CACHE''). 
       %the bold function (``ext4\_sync\_file'') is identified as the root of divergence.
       }
    }
    \label{fig:casefdatasync}
\end{figure*}

==> case-trim.tex <==
\section{Case Study III: \texttt{TRIM}}
\label{sec:case-trim}
%\vspace{-0.1in}

%In practice, because of the lack of multi-layer diagnosis support, 
%the Algolia engineers 
%had to analyze every storage layer deployed
%in their environment, 
%which was ``a terrifying experience" and ended up with
%wrong conclusions~\cite{algolia_blog}.

==> conclude.tex <==
% \vspace{-0.1in}
% \section{Conclusions}
% \label{sec:conclude}
% \vspace{-0.1in}

% We have introduced  \texttt{VDB}
% to help diagnose storage system failures.
% \texttt{VDB} uses cross-layer information and cross-system comparison to narrow down the root cause of failures automatically. Our experiments show that \texttt{VDB} can help reduce the search space by 97 times on average.
% % \
%We have proposed  
%\da{} for better 
%analyzing the reliability
%of the storage software stack.
%\da{} implements three core functionalities,
%including recording the host-device interaction
%for diagnosis, emulating realistic 
%failure device behavior for testing 
%and enhancing the failure handling capability
%of storage software, and predicting 
%the potential unreliable semantics in storage
%software.
%By implementing the core functionalities 
%at the device layer, \da{} minimizes
%the disturbance on the target systems
%and achieves high portability. 


%texttt{VDB} uses virtualization to 
%collect device commands without dependency on the kernel or special hardware, and map the commands to the host side operations to enable cross-layer and cross-system comparison analysis.
%,
%which can arrow down the potential root cause of the failure automatically.
%support unmodified software stack encapsulate the target storage software stack 
%Moreover,
%based on the observation that failures do not always occur under the same workload due to different environment,
%we use a normal system as a reference to automatically 
%narrow down the potential root cause of the failure.
%Our experiments on 12 real-world failure cases show that \texttt{VDB} 
%which can help narrow down the search space of root cause 
%effectively, with an average of 97 times reduction. %



==> perf.tex <==
\vspace{-0.1in}
\subsection{Overhead}
\label{sec:perf}
\vspace{-0.1in}
%Running tracing tools would impact an application's performance and also require space to store the logs. 
%In this section, we individually study the runtime and space overhead that resulted while collecting traces through DevAgent and HostAgent. 
In this section, we study the runtime and space overhead 
of \texttt{VDB}. %, focusing on 
% resulted while collecting traces through DevAgent and HostAgent. 
We use  standard workloads  \textit{varmail}, \textit{webproxy} and \textit{fileserver} from  Filebench~\cite{filebench}  for this set of experiments.  
The parameters are listed in Table~\ref{tab:bench-params},
which are similar to those used in previous work.
%To perform these experiments we have chosen varmail, webproxy and fileserver from the Filebench benchmarking test suite
% \cite{filebench}. 
%The configurations for these workloads are mentioned in Table~\ref{tab:bench-params}.

\begin{table}[tb]
    \begin{center}
    \begin{tabular}{c|c|c|c|c}
    \hline
    \# of  & Mean dir. & Mean file & \# of & Mean IO\\
    files & width & size & threads & size\\
    \hline
    \hline
    1000 & 10 & 16 KB & 1 & 16 KB\\
    \hline
    \end{tabular}
    \end{center}
    \vspace{-0.2in}
    \caption{
    {\bf Filebench Parameters.}
   % {\it This table 
    %summarizes the results of diagnosing XXX failure cases. It 
   % shows the parameters used to setup Filebench benchmark.}
    }
    \label{tab:bench-params}
    \end{table}

\begin{figure}[tb]
    \begin{center}
           \includegraphics[scale=0.22]{./figure/scsiruntime.png}
    \end{center}
    \vspace{-0.25in}
    \caption{
        {\bf Runtime overhead for collecting SCSI commands}. 
     %   {\it This figure shows the normalized runtime overhead resulted while running DevAgent and DevAgent with HostAgent.}
     {\it This figure shows the normalized runtime under three workloads with DevAgent/HostAgent enabled.}
    }
    \label{fig:scsiruntime}
\end{figure}

% \begin{figure}[tb]
%     \begin{center}
%            \includegraphics[scale=0.26]{./figure/nvmeruntime.png}
%     \end{center}
%     %\vspace{-0.15in}
%     \caption{
%         {\bf Runtime overhead for collecting NVMe traces}. 
%         {\it This figure shows the normalized runtime under three workloads with DevAgent/HostAgent enabled. }    }
%     \label{fig:nvmeruntime}
% \end{figure}

\vspace{-0.1in}

\subsubsection{Runtime Overhead}
\label{sec:runtime}
\vspace{-0.1in}

%Fig.\ref{fig:scsiruntime} and \ref{fig:nvmeruntime} show the runtime resulted while the workloads with DevAgent and DevAgent with HostAgent tracers. From the graphs it is obvious that HostAgent results in a severe performance overhead, while DevAgent has negligible impact. It can also be observed that the overhead is relatively higher when collecting NVMe traces. From our experiments we observe that DevAgent captures a lot of NVMe commands at the device layer when compared to the number of SCSI commands. 

% Figure~\ref{fig:scsiruntime} and Figure~\ref{fig:nvmeruntime}  
% show the workload runtime  on SCSI and NVMe devices, respectively.
% In both cases, the DevAgent incurs negligible overhead, while 
% the overhead of HostAgent is noticeable.
% % (e.g., 5.4\% under \textit{varmail}).
% This is mainly because the HostAgent need to generate a large kernel function call tree.
% Overall, the runtime overhead is small (e.g., max 10.6\% 
% under \textit{fileserver} on NVMe in Figure~\ref{fig:nvmeruntime}).


Figure~\ref{fig:scsiruntime} 
shows the workload runtime  with a SCSI device in \texttt{VDB}.
We can see that DevAgent incurs negligible overhead, while 
the overhead of HostAgent is noticeable.
(e.g., 5.4\% under \textit{varmail}).
This is mainly because the HostAgent generates a large kernel function call tree.
Overall, the runtime overhead is small. The results on the NVMe device is similar.
% (e.g., max 10.6\% 
%under \textit{fileserver} on NVMe in Figure~\ref{fig:nvmeruntime}).

\vspace{-0.1in}
\subsubsection{Space Overhead}
\label{sec:space}
\vspace{-0.1in}

%Tab.~\ref{tab:space-overhead} shows the space overhead required to store the traces from DevAgent and HostAgent. Since \texttt{ftrace} collects the function call graph info of the kernel, it is expected to have huge trace footprint for the runtime of the workload. Since we were running our experiments over QEMU, we had to enable \texttt{VIRTIO\_FS} feature and store these traces over the host machine. This was also another reason on why we have chosen to run the workload with small parameter values. 
Table~\ref{tab:space-overhead} shows the space overhead for storing the traces from DevAgent (DA) and HostAgent (HA). 
The traces of HostAgent are  larger than that of DevAgent
because  HostAgent needs to store the kernel function call tree.
%Also, since we were running our experiments over QEMU, we had to enable \texttt{VIRTIO\_FS} feature and store these traces over the host machine. This was also another reason on why we have chosen to run the workload with small parameter values. 
Overall, we find the overhead acceptable. % in the experiments.

\begin{table}[tb]
    \begin{center}
    \begin{tabular}{c|c|c|c|c}
    \hline
   % \multirow{2}{*}{Workload}  & \multicolumn{2}{c|}{SCSI} & \multicolumn{2}{c}{NVMe} \\
       {Workload}  & \multicolumn{2}{c|}{SCSI} & \multicolumn{2}{c}{NVMe} \\
    \cline{2-5}
     & {DA} & {HA}  & {DA} & {HA} \\
    \hline
    \hline
    {varmail}     & \small{1.69 MB} & \small{1.54 GB} & \small{94 MB}  & \small{3.65 GB} \\
    {webproxy} & \small{7.7 KB}    & \small{2.5 GB}    & \small{128 KB}  &  \small{3.6 GB} \\
    {fileserver}  & \small{5.4 KB}    & \small{3.3 GB}   & \small{136.8 KB}  &  \small{3.5 GB} \\
    \hline
    \end{tabular}
    \end{center}
    \vspace{-0.2in}
    \caption{
    {\bf Space Overhead.}
    {\it This table 
    %summarizes the results of diagnosing XXX failure cases. It 
    shows the space overhead of DevAgent (DA) and HostAgent (HA).  %for storing commands from SCSI and NVMe devices.
    }
    }
    \label{tab:space-overhead}
    \end{table}




==> result.tex <==
%\vspace{-0.15in}
\subsection{Case Study I:~\texttt{e2fsck}}
\label{sec:e2fsck}



In this subsection, we apply the testing method to  study \texttt{e2fsck}.
As discussed in \S\ref{sec:background-undo},  \texttt{e2fsck} has recently added 
the  undo logging support. 
 For clarity, we name the original version without undo logging as  \texttt{e2fsck},
 and the version with undo logging as  \texttt{e2fsck-undo}.
%with and without the {undo} logging, respectively.
%Surprisingly, we observe similar unrecoverable corruptions in both cases.
%In other words, the current {undo} logging {cannot} prevent further damages caused
%by an interrupted check. Due to space limit, 
%we only present the results~\textit{with undo logging} in this section\footnote{
%The results of~\texttt{e2fsck} without undo logging can be found in our preliminary report~\cite{our_hotStorage13}.
%}.
%\fixme{update all numbers with undo logging}

We use  175 Ext4 test images from  \texttt{e2fsprogs}  v1.43.1~\cite{e2fsprogs} as inputs to trigger the checker. % \fixme{175 Ext2/3/4?}. %~\texttt{e2fsck}.
The sizes of these images range from 8MB to 128MB, and 
the file system block size is 1KB. %on all these images is 1KB. 
To emulate faults on storage systems with different atomic units, 
we inject faults
at two granularities:  512B and 4KB.  
In other words, we interrupt~\texttt{e2fsck} after every 512B or 4KB  of an I/O transfer command. 
Since the file system block is 1KB, we do not break file system blocks when injecting faults at the 4KB granularity. 

First, we study \texttt{e2fsck}  using the method in Figure~\ref{fig:workflow}a.
As described in \S\ref{sec:workflow}, for each fault injected (i.e., each interruption) we run \texttt{e2fsck} again and generate one repaired image.
From one test image we usually generate multiple repaired images because the repairing procedure usually requires updating 
multiple file system blocks.
For example, to fix the test image ``\texttt{f\_noroot}'' (image with no root directory) from \texttt{e2fsprogs},  \texttt{e2fsck} needs to update four 1KB blocks, which generates eight interrupted images (and consequently repaired images) when faults are injected after every 512B. 
%Among these 8 images, 4 images have reported "file content corruption" and other 4 have reported "misplacement of files".  
Table~\ref{tab:num_images} summarizes the total number of repaired images generated 
from the 175 test images at the two granularities.
%We can see that with the finer grain of fault injection (i.e., 512B), more repaired images are generated because the repairing procedure is 
We can see that  the 512B case leads to more repaired images (i.e., 25,062) because the repairing procedure is 
 interrupted more frequently. 


\begin{table}[tb]
\begin{center}
\begin{tabular}{c|c|c}
\hline
{\# of Ext4} & {Fault injection} & {Total \# of} \\
{test images} & {granularity}  & {repaired images} \\
\hline
\hline
175 & 512 B & 25,062  \\
175 & 4 KB & 3,195 \\
\hline
\end{tabular}
\end{center}
\vspace{-0.2in}
\caption{
{\bf Total number of repaired images.} 
{\it This table shows the number of repaired images generated from 175 Ext4 test images at two fault injection granularities.}
}
\label{tab:num_images}
\end{table}


\begin{table}[tb]
\begin{center}
\begin{tabular}{c|c|c}
\hline
{Fault injection} & \multicolumn{2}{c}{{\# of images reporting corruptions}} \\
\cline{2-3}
{granularity} & {test images}  & {repaired images} \\
\hline
\hline
512 B & 34 & 240  \\
4 KB & 17 & 37 \\
\hline
\end{tabular}
\end{center}
\vspace{-0.2in}
\caption{
%{\bf Number of Ext4 images reporting corruptions under two fault injection granularities.}
{\bf Number of images reporting corruptions. }
 {\it This table shows the number of Ext4 test images and repaired images reporting 
 corruptions at two fault injection granularities.}
%\fixme{add  undo logging results for the 17 or 34 images}
}
\label{tab:num_corruptions}
\end{table}

\begin{table}[t]
\begin{center}
\begin{tabular}{c|c|c}
\hline
{Corruption Type} & 512 B & 4 KB \\
\hline
\hline
{cannot mount} & 41 & 3 \\
{file content corruption} & 107 & 10 \\
{misplacement of files} & 82 & 23 \\
others & 10 & 1\\
\hline
Total & 240 & 37\\
\hline
\end{tabular}
\end{center}
\vspace{-0.2in}
\caption{
%\small{
%Number of  repaired images reporting each type of corruptions under two fault injection granularities.
{\bf Classification of corruptions.}
{\it This table shows the number of  repaired images reporting each type of corruptions at two fault injection granularities.}
}
\label{tab:normalresult}
\end{table}


By comparing with the reference image (Figure~\ref{fig:workflow}a), we can verify if a repaired image
contains unrecoverable corruptions or not. If at least one repaired image contains such corruption, we mark the corresponding test image
as reporting corruption, too. 
Table~\ref{tab:num_corruptions}  shows the numbers of test images and repaired images reporting  corruptions.
We can see that at the 512B granularity, more images have corruptions (e.g., 34  $>$ 17). This is because the updates are broken into smaller pieces,
and thus it is more challenging to maintain consistency when interrupted.


To further understand the severeness of the corruptions, 
we examine the symptoms  in  details and classify them into four types, including:
(1) \textit{cannot mount}; % file systems;
(2) \textit{file content corruption}; 
(3) \textit{misplacement of files} (e.g., a file is either in the``lost+found'' folder or completely missing)
(4) \textit{others} (e.g.,  showing ``???'' after an {\tt ls} command).  
Table~\ref{tab:normalresult} shows the number of  repaired images reporting each type of corruptions.
We can see that \textit{file content corruption} and \textit{misplacement of files}
are most common. Also, even at a fault injection granularity bigger than the file system block (i.e., 4KB $>$ 1KB), we still observe
three cases where the whole file system volume becomes not mountable  (i.e., ``cannot mount''). %becomes {unmountable}.
%Note that all these corruptions were observed 
%after running the checker again without interruption, 
%which means they cannot be recovered by the existing checker. 



\begin{table}[tb]
\begin{center}
\begin{tabular}{c|c|c}
\hline
{Fault injection} & \multicolumn{2}{c}{{\# of images reporting corruptions}} \\
\cline{2-3}
{granularity} & { e2fsck}  & { e2fsck-undo} \\
\hline
\hline
512 B & 34 & 34  \\
4 KB & 17 & 15 \\
\hline
\end{tabular}
\end{center}
\vspace{-0.2in}
\caption{
{\bf Comparison of e2fsck and e2fsck-undo.}
%{\bf Number of images reporting corruptions when testing e2fsck-undo. }
 {\it This table compares the number of test images reporting 
 corruptions under {e2fsck} and {e2fsck-undo}.}
 % two fault injection granularities when undo logging is enabled.}
%\fixme{add results}
}
\label{tab:num_corruptions-logging}
\end{table}

Next, to see if the undo logging can avoid the corruptions, % caused by \texttt{e2fsck}, 
we use the method in Figure~\ref{fig:workflow}b to study \texttt{e2fsck-undo}.
We focus on the test images  which report
corruptions when testing \texttt{e2fsck} (i.e., the 34 and 17 test images in Table~\ref{tab:num_corruptions}).% at the 4 KB fault injection granularity.

Table~\ref{tab:num_corruptions-logging} compares the number of test images reporting 
 corruptions under \texttt{e2fsck} and \texttt{e2fsck-undo}. 
 Surprisingly, we observe a similar amount of corruptions.
 %at both granularities \fixme{wait for result}. 
 For example, all 34 images which report corruptions when testing \texttt{e2fsck} at the 512B granularity 
 still report corruptions under \texttt{e2fsck-undo}.
 We defer the analysis of the root cause to \S\ref{sec:why}.


